Optimization Helps Scheduling Nursing Staff at the Long-Term Care Homes of the City of Toronto

The City of Toronto Long Term Care Homes & Services (LTCH&S) division is one of the largest providers of long-term care in the Canadian province of Ontario, providing care to 2,640 residents at 10 homes across Toronto. Our collaboration with LTCH&S was initiated to facilitate the increasingly challenging task of scheduling nursing staff and reduce high absenteeism rate observed among the part-time nurses. We developed a spreadsheet-based scheduling tool to automate the generation of schedules and incorporate nurses' preferences for different shifts into the schedules. At the core of the scheduling tool is a hierarchical optimization model that generates a feasible schedule with the highest total preference score while satisfying the maximum possible demand. Feasible schedules had to abide by a set of complex seniority requirements which prioritized more senior nurses when allocating the available shifts. Our scheduling tool was implemented in a 391-bed home in Toronto. The tool allowed nursing managers to generate feasible schedules within a fraction of an hour, in contrast to the status-quo manual approach which could took up to tens of hours. In addition, the schedules successfully accounted for preferences with on average above 94% of the allocated shifts ranked as most preferred.

==> NotUsed/Outline.tex <==
\subsection{Introduction}
    \begin{enumerate}
	\item Motivation: Discuss the Current Process and the Problems the Division is Facing
			\begin{enumerate}
				\item Explain how schedules are generated currently and the explain the two major issues with the current process. 
				\item (1) the time required to build an initial working schedule, and the amount of revision required after schedule posting. The lengthy time required to build an initial feasible schedule is due to the long scheduling horizon, the large number of nurses to be scheduled, and restrictive seniority rules. The large amount of revision is due to late leave requests, call ins, etc.
				\item (2) The issue of high absenteeism among part-time nurses; preferences are not taken into account.
			\end{enumerate}
	\item Define the problem type
			\begin{enumerate}
				\item This problem is a unique case of the Nurse Scheduling Problem (NSP) with a restrictive seniority rule and uniform demand
			\end{enumerate}
	\item Discuss Literature with similar implementation approaches
			\begin{enumerate}
				\item Discuss papers that utilize a spreadsheet implementation 
			\end{enumerate}
	\item Provide a short summary of the collaboration, objectives; and the proposed solution approach and its implementation.
			\begin{enumerate}
			\item Provide background information on the relationship between the authors and the institution.
			\item Objectives and requirements of the solution (high-level description) that were critical to implementation
			\item Summary of the technical approach and its positioning in the literature
			\begin{enumerate}   
				\item We have addressed the problem by developing a model which automates the generation of schedules. This model has two main components; a two-stage integer programming model and a heuristic algorithm. 
				\item We have also introduced preference based shift scheduling in an attempt to reduce call ins.
			\end{enumerate}
			\item Summary of the implementation and outcomes. 	
			\end{enumerate}
	\item Discuss the structure of the paper.
	\end{enumerate}
	
\subsection{Problem Description}
	\begin{enumerate}
	\item Discuss Literature with similar problems and approaches
		\begin{enumerate}
			\item Papers that also deal with maximizing nurse preference in an NSP \cite{jafari2015maximizing}
			\item Different solution approaches to the NSP; Binary Goal Programming, Metaheuristics (Simulated Annealing \cite{jafari2015maximizing}, Genetic Algorithms)
			\item Papers that also deal with seniority within scheduling problems
		\end{enumerate}
	\item Describe the unique features of our problem [MB: Maybe not as a separate paragraph, but inside the above paragraphs, as needed.]
		\begin{enumerate}
			\item Combining a highly restrictive seniority rule (The Armstrong rule), with maximizing nurse preferences
		\end{enumerate}
	
	\item Objective (satisfy demand with a feasible schedule that achieves a high total preference): generate schedules for 6-week planning periods that describe shifts where nurses of different types will work to satisfy a (deterministic) demand. In addition wanted to allocate shifts such that the preferences are maximized. 
	\item Requirements:
			\begin{enumerate}
				\item The weekend, max out, demand, back to back, and seniority requirements
				\item seniority requirements: the Armstrong rule 
				\item Implementation and automation requirements. (e.g., allow for updating staff availability and preference, time-considerations, etc.)
			\end{enumerate}
	 \end{enumerate}
	 
\subsection{Solution Approach}
		\begin{enumerate}
		\item Approximate Integer Programming Model
		\begin{enumerate}
		    \item Describe the IP model and the heuristic using a diagram
			\item Discuss the Integer programming model (for each stage objectives, constraints, decision variables, input data and output)
			\begin{enumerate}
				\item Discuss the inputs to the model
				\item Discuss the objective of each stage of the model 
				\item Discuss how the constraints are used to obtain optimal solutions for the case where the demand is less than the nominal (8,6,4,3) values of the armstrong rule, and an infeasible starting point for the heuristics when the demand is at or greater than the nominal values of the amstrong rule
				\item Describe the outputs of the IP
			\end{enumerate}
			\item describe the heuristic; its input and output
			\begin{enumerate}
				\item Discuss the inputs from the IP required for the algorithm
				\item Discuss how the heuristic obtains feasible solutions when the demand is at or greater than the nominal (8,6,4,3) values of the armstrong rule
				\item Describe the stopping criteria of the algorithm
			\end{enumerate}
		\end{enumerate}
		\item Describe the User Interface
		\begin{enumerate}
				\item Describe how the user interface enables data collection and storage
				\item Describe how the user interface enables the formulation of the optimization models, interaction with the OpenSolver and execution of the heuristic algorithm
				\item Describe how the user interface formats the schedule output into a readable format and provide an example
		\end{enumerate}
		\item Exact Integer Programming Model
		\end{enumerate}
		
\subsection{Implementation and Results}
	\begin{enumerate}
	\item Pilot setting and details
		\begin{enumerate}
			\item Discuss the process for collecting availability and vacation data
			\item The user who executes the process is mentioned
			\item The software and hardware components used to execute the model are discussed
		\end{enumerate}
	\item Discussion of implementation dates, timelines, and results
		\begin{enumerate}
			\item Pilots at Cummer Lodge 2nd Floor (2 Units, ~80 employees)
				\begin{enumerate}
					\item 1st Pilot, Schedule Posted: Dec 4th/2019, Cycle: December 18th/2019 - February 28th/2020
					\item 2nd Pilot, Schedule Posted: January 15th/2020, Cycle: February 29th/2020 - March 3rd/2020
					\item 2rd Pilot, Schedule Posted: February 26th/2020, Cycle: March 11th/2020 - April 21rd/2020
				\end{enumerate}
			
			\item Pilots at Cummer Lodge - Whole Home (7 Units, ~300 nurses)	
				\begin{enumerate}
					\item 4th Pilot, Schedule Posted: April 8th/2020, Cycle: April 22nd/2020 - June 3rd/2020
				\end{enumerate}
			
			\item Discussion of City Wide Implementation (10 Homes, ~2200 nurses)	
				\begin{enumerate}
					\item Scalable User Interface Required
				\end{enumerate}
				
		\end{enumerate}
	
	
	\item Discuss Challenges with Implementation
		\begin{enumerate}
			\item Issues with Data Collection and Input
			\item Process related Challenges
			\item Minor manual adjustments required to obtain a feasible solution
		
		\end{enumerate}
	
	
	\item Quantifiable and Non-Quantifiable benefits Discussed
		\begin{enumerate}
			\item Discuss the quantifiable benefits 
				\begin{enumerate}
					\item Reduction in Lead Time for Schedule Generation
					\item Financial/Time Related Savings
					\item Reduction in Call-In Rates
					\item Turn over rates
				\end{enumerate}
		
			\item Discuss the non-quantifiable benefits 
				\begin{enumerate}
					\item Nurse Satisfaction
					\item Bias free schedules 
				\end{enumerate}	
			
		\end{enumerate}

	\end{enumerate}


\subsection{Conclusion}
	
	\begin{enumerate}
		\item Summary of the models proposed in the paper
		\item Discuss the limitations of the approach
		\item Discuss the ongoing implementation of the solution
		\item Discussion of potential future applications (expansions) of the model			
	\end{enumerate}
